Graph Positional and Structural Encoder

Positional and structural encodings (PSE) enable better identifiability of nodes within a graph, rendering them essential tools for empowering modern GNNs, and in particular graph Transformers. However, designing PSEs that work optimally for all graph prediction tasks is a challenging and unsolved problem. Here, we present the Graph Positional and Structural Encoder (GPSE), the first-ever graph encoder designed to capture rich PSE representations for augmenting any GNN. GPSE learns an efficient common latent representation for multiple PSEs, and is highly transferable: The encoder trained on a particular graph dataset can be used effectively on datasets drawn from markedly different distributions and modalities. We show that across a wide range of benchmarks, GPSE-enhanced models can significantly outperform those that employ explicitly computed PSEs, and at least match their performance in others. Our results pave the way for the development of foundational pre-trained graph encoders for extracting positional and structural information, and highlight their potential as a more powerful and efficient alternative to explicitly computed PSEs and existing self-supervised pre-training approaches. Our framework and pre-trained models are publicly available at https://github.com/G-Taxonomy-Workgroup/GPSE. For convenience, GPSE has also been integrated into the PyG library to facilitate downstream applications.

==> tables/abl_conv_layers_vn.tex <==
\begin{table}[!htp]\centering
% \scriptsize
\fontsize{8.5pt}{8.5pt}\selectfont
\renewcommand{\arraystretch}{1.2}
\setlength\tabcolsep{6pt} % default value: 6pt
\caption{Virtual node, convolution type, and layers ablation using 5\% MolPCBA for training. \todo{Put it side by side with E4}}\label{tab:abl_conv_layers_vn}
% \begin{tabular}{@{}ccccc@{}}
\begin{tabular}{@{\extracolsep{10pt}}ccccc@{}}
\toprule
&\multicolumn{2}{c}{\method (GatedGCN)} &\multicolumn{2}{c}{\method (GIN)} \\
\cmidrule{2-3}
\cmidrule{4-5}
Layers &VN & no VN &VN & no VN \\
\midrule
5 &0.8387 &0.6982 &0.4879 &0.1347 \\
10 &0.9585 &0.8353 &0.5156 &0.2476 \\
15 &0.9716 &0.9231 &0.5887 &0.2523 \\
20 &0.9778 &0.9478 &0.6095 &0.2743 \\
30 &0.9806 &0.9559 &0.4149 &0.3740 \\
40 &0.9782 &0.9459 &0.5420 &0.3968 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/abl_depth.tex <==
\centering
\scriptsize
\begin{tabular}{@{}ll@{}}
\toprule
Num layers & R2 \\ \midrule
10                  & 0.9814      \\
15                  & 0.9848      \\
20                  & 0.9869      \\
25                  & 0.9889      \\
30                  & 0.9893      \\
\textbf{40}                  & \textbf{0.9913}      \\ \bottomrule
\end{tabular}
\caption{Model depth}\label{tab:abl_depth}

==> tables/abl_models_vn.tex <==
\begin{table}[!htp]\centering
\caption{Message-passing type \& Virtual node experiments}\label{tab:abl_models_vn}
\scriptsize
\begin{tabular}{@{}lll@{}}
\toprule
                 & \multicolumn{2}{c}{R2 score for dataset}                   \\ \midrule
Model            & ogbg-molhiv (10-layer) & ZINC-full (20-layer) \\ \midrule
\textbf{ResGatedGCN}      & \textbf{0.9816}                 & \textbf{0.979}                \\
ResGatedGCN-NoVN & 0.9009                 & 0.9466               \\
GATv2            & 0.9375                 & 0.9565               \\
GIN              & 0.6065                 & 0.4121               \\
GCN              & 0.08482                & -0.01434             \\ \bottomrule
\end{tabular}
\end{table}

==> tables/abl_staging.tex <==
\centering
\scriptsize
\begin{tabular}{@{}ll@{}}
\toprule
Staging    & Test R2 \\ \midrule
\textbf{skipsum}    & \textbf{0.8154}  \\
stack      & 0.731   \\
skipconcat & 0.6932  \\ \bottomrule
\end{tabular}
\caption{Staging}\label{tab:abl_staging}

==> tables/abl_width.tex <==
\centering
\scriptsize
\begin{tabular}{@{}ll@{}}
\toprule
Dim inner & Test R2 \\ \midrule
128       & 0.9653  \\
256       & 0.9701  \\
512       & 0.9784  \\
\textbf{1024}      & \textbf{0.982}   \\ \bottomrule
\end{tabular}
\caption{Model width}\label{tab:abl_width}

==> tables/molnet_rebuttal.tex <==
\begin{table}[!htp]\centering
\caption{Performance on MoleculeNet small datasets (scaffold test split), evaluated in AUROC (\%) $\uparrow$. \textcolor{dark2pink}{Red} indicates worse than baseline performance.}\label{tab:molnet}
\scriptsize
\vspace{3pt}
\begin{tabular}{lcccccc}\toprule
&\textbf{BBBP} &\textbf{BACE} &\textbf{Tox21} &\textbf{ToxCast} &\textbf{SIDER} \\
\midrule
No pre-training (baseline) &65.8 ± 4.5 &70.1 ± 5.4 &74.0 ± 0.8 &63.4 ± 0.6 &57.3 ± 1.6 \\
\midrule
Self-supervised pre-trained &68.8 ± 0.8 &79.9 ± 0.9 &\textbf{76.7 ± 0.4} &64.2 ± 0.5 &61.0 ± 0.7 \\
GraphCL pre-trained &69.7 ± 0.7 &75.4 ± 1.4 &\textcolor{dark2pink}{73.9 ± 0.7} &\textcolor{dark2pink}{62.4 ± 0.6} &60.5 ± 0.9 \\
InfoGraph pre-trained &66.3 ± 0.6 &\textcolor{dark2pink}{64.8 ± 0.8} &\textcolor{dark2pink}{68.1 ± 0.6} &\textcolor{dark2pink}{58.4 ± 0.6} &\textcolor{dark2pink}{57.1 ± 0.8} \\
JOAOv2 pre-trained &66.4 ± 0.9 &\textcolor{dark2pink}{67.4 ± 0.7} &\textcolor{dark2pink}{68.2 ± 0.8} &\textcolor{dark2pink}{57.0 ± 0.5} &59.1 ± 0.7 \\
MoleBERT &71.9 ± 1.6 &80.8 ± 1.4 &\textbf{76.8 ± 0.5} &64.3 ± 0.2 &\textbf{62.8 ± 1.1} \\
GraphMAE &72.0 ± 0.6 &83.1 ± 0.9 &75.5 ± 0.6 &64.1 ± 0.3 &60.3 ± 1.1 \\
GraphLoG &\textbf{72.5 ± 0.8} &\textbf{83.5 ± 1.2} &75.7 ± 0.5 &63.5 ± 0.7 &61.2 ± 1.1 \\
GraphLoG (Feature extractor) &\textcolor{dark2pink}{65.6 ± 1.0} &82.5 ± 1.2 &\textcolor{dark2pink}{73.2 ± 0.5} &63.6 ± 0.4 &60.9 ± 0.7 \\
\midrule
GPSE augmented (MolPCBA) &66.4 ± 0.1 &78.3 ± 2.7 &74.9 ± 0.4 &\textbf{65.7 ± 0.6} &61.5 ± 0.8\\
GPSE augmented (MNIST) &67.5 ± 1.3 &79.0 ± 1.4 &76.2 ± 0.7 &\textbf{66.0 ± 0.6} &61.1 ± 0.6\\
\bottomrule
\end{tabular}
\end{table}

==> tables/node_bench.tex <==
\begin{table}[!htp]\centering
% \vspace{-10pt}
\caption{OOD transferability to OGB node classification benchmarks.}\label{tab:nodebench}
% \scriptsize
\tiny
\setlength\tabcolsep{5pt} % default value: 6pt
\tiny
\begin{tabular}{lcccc}\toprule
& &\textbf{arXiv} &\textbf{Proteins} \\
& +\method?&\textbf{ACC} (\%) $\uparrow$ &\textbf{AUROC} (\%) $\uparrow$ \\
\midrule
GCN     &\xmark &71.74 ± 0.29 &79.91 ± 0.24 \\
        &\cmark &71.67 ± 0.12 &79.62 ± 0.12 \\
% \midrule
SAGE    &\xmark &71.74 ± 0.29 &80.35 ± 0.07 \\
        &\cmark &72.19 ± 0.32 &80.14 ± 0.22 \\
% \midrule
% GIN(E)                  &\xmark &71.82 ± 0.17 &83.70 ± 0.27 \\
%                         &\cmark &71.85 ± 0.09 &83.60 ± 0.09 \\
% \midrule
GAT(E)v2    &\xmark &71.69 ± 0.21 &83.47 ± 0.13 \\
            &\cmark &72.17 ± 0.42 &83.51 ± 0.11 \\
% GCN~\citep{hu2020open}   &\xmark &71.74 ± 0.29 &79.91 ± 0.24 \\
%                         &\cmark &71.67 ± 0.12 &79.62 ± 0.12 \\
% % \midrule
% SAGE~\citep{hu2020open}  &\xmark &71.74 ± 0.29 &80.35 ± 0.07 \\
%                         &\cmark &72.19 ± 0.32 &80.14 ± 0.22 \\
% % \midrule
% % GIN(E)                  &\xmark &71.82 ± 0.17 &83.70 ± 0.27 \\
% %                         &\cmark &71.85 ± 0.09 &83.60 ± 0.09 \\
% % \midrule
% GAT(E)v2~\citep{brody2021attentive}                &\xmark &71.69 ± 0.21 &83.47 ± 0.13 \\
%                         &\cmark &72.17 ± 0.42 &83.51 ± 0.11 \\
\midrule
\textit{Best of above}  &\xmark &71.74 ± 0.29 &83.47 ± 0.13 \\
                        &\cmark &\textbf{72.19 ± 0.32} &\textbf{83.51 ± 0.11} \\
\bottomrule
\end{tabular}
%\vspace{-0.1in}
\end{table}


% \begin{table}[!htp]\centering
% \caption{OGB node classification benchmarks}\label{tab:nodebench}
% \scriptsize
% \begin{tabular}{lcccc}\toprule
% &+GPSE?&\textbf{ogbn-arXiv} &\textbf{ogbn-proteins} \\
% & &\textbf{ACC} $\uparrow$ &\textbf{AUROC} $\uparrow$ \\
% \midrule
% GCN~\cite{hu2020open} & \xmark &71.740 ± 0.290 &72.510 ± 0.350 \\
% GraphSAGE~\cite{hu2020open} &\xmark &71.740 ± 0.290 &77.680 ± 0.200 \\
% GIN &\xmark &71.56 ± 0.233 &xx.xxx ± 0.xxx \\
% GATv2 &\xmark &71.53 ± 0.170 &82.287 ± 0.192 \\
% \midrule
% GCN+GPSE &\cmark &71.47 ± 0.282 &xx.xxx ± 0.xxx \\
% GraphSAGE+GPSE &\cmark &71.69 ± 0.225 &xx.xxx ± 0.xxx \\
% GIN+GPSE &\cmark &71.99 ± 0.338 &xx.xxx ± 0.xxx \\
% GATv2+GPSE &\cmark &72.23 ± 0.321 &xx.xxx ± 0.xxx \\
% \bottomrule
% \end{tabular}
% \end{table}

==> tables/node_bench_full.tex <==
\begin{table}[htp]
\captionsetup{width=.5\linewidth}
\centering
\caption{Extended results for Table~\ref{tab:nodebench}: OOD transferability to OGB node classification benchmarks.}\label{tab:nodebench_full}
% \scriptsize
% \tiny
\setlength\tabcolsep{5pt} % default value: 6pt
\begin{tabular}{lcccc}\toprule
& &\textbf{arXiv} &\textbf{Proteins} \\
& +\method?&\textbf{ACC} (\%) $\uparrow$ &\textbf{AUROC} (\%) $\uparrow$ \\
\midrule
GCN     &\xmark &71.74 ± 0.29 &79.91 ± 0.24 \\
        &\cmark &71.67 ± 0.12 &79.62 ± 0.12 \\
% \midrule
SAGE    &\xmark &71.74 ± 0.29 &80.35 ± 0.07 \\
        &\cmark &72.19 ± 0.32 &80.14 ± 0.22 \\
% \midrule
% GIN(E)                  &\xmark &71.82 ± 0.17 &83.70 ± 0.27 \\
%                         &\cmark &71.85 ± 0.09 &83.60 ± 0.09 \\
% \midrule
GAT(E)v2    &\xmark &71.69 ± 0.21 &83.47 ± 0.13 \\
            &\cmark &72.17 ± 0.42 &83.51 ± 0.11 \\

Transformer &\xmark &57.00 ± 0.79 &73.93 ± 1.44 \\
            &\cmark &59.17 ± 0.21 &74.67 ± 0.74 \\

GPS         &\xmark &70.60 ± 0.28 &69.55 ± 5.67 \\
            &\cmark &70.89 ± 0.36 &72.05 ± 3.75 \\

\midrule
\textit{Best of above}  &\xmark &71.74 ± 0.29 &83.47 ± 0.13 \\
                        &\cmark &\textbf{72.19 ± 0.32} &\textbf{83.51 ± 0.11} \\
\bottomrule
\end{tabular}
\vspace{-0.1in}
\end{table}

==> tables/sat_bench.tex <==
\begin{table}[htp]
\captionsetup{width=.5\linewidth}
\centering
\caption{SAT~\citep{sat_chen_2022} comparison of GPSE and RWSE on ZINC. Results averaged over 3 seeds.}\label{tab:satbench}
% \scriptsize
% \tiny
\setlength\tabcolsep{5pt} % default value: 6pt
\begin{tabular}{lcccc}\toprule
&\textbf{ZINC} (subset) &\textbf{ZINC} (subset)\\
&\textbf{MAE} $\downarrow$ &\textbf{MSE} $\downarrow$\\
\midrule
k-ST SAT+\method    &\textbf{0.0830 ± 0.0023} &\textbf{0.0251 ± 0.0040} \\
k-ST SAT+RWSE    &0.1068 ± 0.0053 &0.0584 ± 0.0130 \\
\midrule
k-SG SAT+\method    &\textbf{0.0873 ± 0.0008} &\textbf{0.0277 ± 0.0030} \\
k-SG SAT+RWSE    &0.0900 ± 0.0024 &0.0300 ± 0.0087 \\

\bottomrule
\end{tabular}
\vspace{-0.1in}
\end{table}

==> tables/scaling_law.tex <==
\begin{table}[!htp]\centering
% \scriptsize
\fontsize{8.5pt}{8.5pt}\selectfont
\renewcommand{\arraystretch}{1.2}
\setlength\tabcolsep{6pt} % default value: 6pt
\caption{Training size scaling law for \method on MolPCBA.}\label{tab:scaling_law}
\begin{tabular}{@{}cc@{}}
\toprule
Training size & Overall test R2 ($\uparrow$)\\
\midrule
5\%     & 0.06939 \\
10\%    & 0.04414 \\
20\%    & 0.03579 \\
40\%    & 0.01945 \\
80\%    & 0.01219 \\
\bottomrule
\end{tabular}
\end{table}
